On Thermodynamics and Phase Space of Near Horizon Extremal Geometries

Near Horizon Extremal Geometries (NHEG), are geometries which may appear in the near horizon region of the extremal black holes. These geometries have $SL(2,\mathbb{R})\!\times\!U(1)^n$ isometry, and constitute a family of solutions to the theory under consideration. In the first part of this report, their thermodynamic properties are reviewed, and their three universal laws are derived. In addition, at the end of the first part, the role of these laws in black hole thermodynamics is presented. In the second part of this thesis, we review building their classical phase space in the Einstein-Hilbert theory. The elements in the NHEG phase space manifold are built by appropriately chosen coordinate transformations of the original metric. These coordinate transformations are generated by some vector fields, dubbed "symplectic symmetry generators." To fully specify the phase space, we also need to identify the symplectic structure. In order to fix the symplectic structure, we use the formulation of Covariant Phase Space method. The symplectic structure has two parts, the Lee-Wald term and a boundary contribution. The latter is fixed requiring on-shell vanishing of the symplectic current, which guarantees the conservation and integrability of the symplectic structure, and leads to the new concept of "symplectic symmetry." Given the symplectic structure, we construct the corresponding conserved charges, the "symplectic symmetry generators." We also specify the explicit expression of the charges as a functional over the phase space. These symmetry generators constitute the "NHEG algebra," which is an infinite dimensional algebra (may be viewed as a generalized Virasoro), and admits a central extension which is equal to the black hole entropy.

==> Thesis arXiv v2/fig-AdS2.tex <==
\begin{center}
\hspace*{-3cm}
\subfigure{\includegraphics[width=0.7\textwidth]{AdS2.png}}
\hspace{-7.7cm}
\subfigure{\begin{tikzpicture}[scale=1]
            \draw (1,0.67) node{};
            \fill[darkblue] (0,9.5) circle (0.05cm);
            \fill[darkblue] (-2.5,9.5) circle (0.05cm);
            \draw (0,9.5) node{\includegraphics[width=0.1\textwidth]{Sphere.png}}; 
            \draw[ultra thick,->,>=stealth] (-0.4,7.72) -- (0,9.5);
            \draw (1,9.5) node{$\mathcal{H}$};
            \draw (0.2,8.4) node{${\mrn}_{_\mathcal{H}}^a$};
            \draw (-2.5,9.5) node[anchor=south]{$(t,r)$};
            \draw[ultra thick,->,>=stealth] (-1.7,7.78) -- (-2.5,9.5);
            \draw (-1.7,8.7) node{${\mrn}^a$};
           \end{tikzpicture}
}
\end{center}
\caption{\footnotesize The $AdS_2$ sector of a NHEG is a $2$-dim surface which can be immersed in $\mathbb{R}^{2,1}$. Its Poincar\'e patch is  parametrized by the coordinates $(t,r)$. The vector $\mrn^a$  is a vector connecting the origin to the point $(t,r)$. At each point of the surface, identified by $(t_{_\mathcal{H}},r_{_\mathcal{H}})$, there is a $d\!-\!2$ dimensional closed and smooth manifold, denoted by $\mathcal{H}$. It is depicted in the figure, intuitively and schematically .  The $\mrn^a$  which points to $(t_{_\mathcal{H}},r_{_\mathcal{H}})$ is labelled by $\mrn_{_\mathcal{H}}^a$. Although the figure is drawn by intuition, but it might be misleading: The NHEG is not generically a direct product as $AdS_2\times \mathcal{H}$.}

==> Thesis arXiv v2/fig-isometry-BH.tex <==
\begin{center}
\subfigure[]{\label{fig ext BH}\includegraphics[width=0.45\textwidth]{BlackholeNH.jpg}}
\hspace{1cm}
\subfigure[]{\label{fig ext BH NH}\includegraphics[width=0.45\textwidth]{BlackholeNH2.png}}
\end{center}
\caption{\footnotesize (a) A schematic of a rotating extremal BH. It is in black, because it does not have any radiation. It has $\mathbb{R}\times U(1)^n$ isometry. (b) A schematic of near horizon region of that extremal BH. The isometry enhances to $SL(2,\mathbb{R})\times U(1)^n$.}

==> Thesis arXiv v2/fig-isometry-earth.tex <==
\begin{center}
\subfigure[]{\label{fig earth}\includegraphics[width=0.45\textwidth]{earth.jpg}}
\hspace{1cm}
\subfigure[]{\label{fig earth land}\includegraphics[width=0.45\textwidth]{earthland.jpg}}
\end{center}
\caption{\footnotesize (a) The earth is a planet with spherical isometry. The group of the isometry is $SO(3)$. (b) Close to the surface of the earth, the isometry changes to $\mathbb{R}^2\times U(1)$. It is translations in the  depicted desert, and rotation around an axis perpendicular to the surface of desert. (Photo taken by Fatemeh Bagheri,  Iran.)}

==> Thesis arXiv v2/pgflibraryam.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter

% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{133}\def\@pgfornamentY{48}%  2
\fi%
}%
% appels des motifs 
\def\pgf@@ornament#1{%
\begingroup
\def\i{\pgfusepath{clip}}
\let\o\pgfpathclose
\let\s\pgfusepathqfillstroke
\def\p ##1##2{\pgfqpoint{##1bp}{##2bp}}
\def\m ##1 ##2 {\pgfpathmoveto{\p{##1}{##2}}}
\def\l ##1 ##2 {\pgfpathlineto{\p{##1}{##2}}}
\def\r ##1 ##2 ##3 ##4 {\pgfpathrectangle{\p{##1}{##2}}{\p{##3}{##4}}}
\def\c ##1 ##2 ##3 ##4 ##5 ##6 {%
\pgfpathcurveto{\p{##1}{##2}}{\p{##3}{##4}}{\p{##5}{##6}}}%
\@@input am#1.pgf 
%\@nameuse{pgf@@am@#1}%
\endgroup}%
\makeatother
\endinput   

==> Thesis arXiv v2/pgflibraryvectorian.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter
% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{134}\def\@pgfornamentY{48}%  2
\or\def\@pgfornamentX{130}\def\@pgfornamentY{65}%  3
\or\def\@pgfornamentX{133}\def\@pgfornamentY{133}% 4
\or\def\@pgfornamentX{129}\def\@pgfornamentY{146}% 5
\or\def\@pgfornamentX{134}\def\@pgfornamentY{148}% 6
\or\def\@pgfornamentX{136}\def\@pgfornamentY{135}% 7
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 8
\or\def\@pgfornamentX{79}\def\@pgfornamentY{105}% 9
\or\def\@pgfornamentX{80}\def\@pgfornamentY{99}%  10
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  11
\or\def\@pgfornamentX{136}\def\@pgfornamentY{136}% 12
\or\def\@pgfornamentX{136}\def\@pgfornamentY{236}% 13
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  14
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  15
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  16
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  17
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  18
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  19
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  20
\or\def\@pgfornamentX{70}\def\@pgfornamentY{58}%  21
\or\def\@pgfornamentX{34}\def\@pgfornamentY{61}%  22
\or\def\@pgfornamentX{68}\def\@pgfornamentY{55}%  23
\or\def\@pgfornamentX{79}\def\@pgfornamentY{76}%  24
\or\def\@pgfornamentX{80}\def\@pgfornamentY{88}%  25
\or\def\@pgfornamentX{59}\def\@pgfornamentY{120}% 26
\or\def\@pgfornamentX{101}\def\@pgfornamentY{98}%  27
\or\def\@pgfornamentX{52}\def\@pgfornamentY{102}% 28
\or\def\@pgfornamentX{65}\def\@pgfornamentY{65}%  29
\or\def\@pgfornamentX{63}\def\@pgfornamentY{64}%  30
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  31
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  32
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  33
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  34
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  35
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  36
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 37
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 38
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 39
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 40
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 41
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 42
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  43
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  44
\or\def\@pgfornamentX{385}\def\@pgfornamentY{64}%  45
\or\def\@pgfornamentX{453}\def\@pgfornamentY{97}%  46
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  47
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  48
\or\def\@pgfornamentX{163}\def\@pgfornamentY{61}%  49
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 50
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 51
\or\def\@pgfornamentX{248}\def\@pgfornamentY{197}% 52
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 53
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 54
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 55
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 56
\or\def\@pgfornamentX{207}\def\@pgfornamentY{103}% 57
\or\def\@pgfornamentX{228}\def\@pgfornamentY{116}% 58
\or\def\@pgfornamentX{204}\def\@pgfornamentY{102}% 59
\or\def\@pgfornamentX{451}\def\@pgfornamentY{189}% 60
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 61
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 62
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 63
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 64
\or\def\@pgfornamentX{132}\def\@pgfornamentY{166}% 65
\or\def\@pgfornamentX{177}\def\@pgfornamentY{175}% 66
\or\def\@pgfornamentX{80}\def\@pgfornamentY{155}% 67
\or\def\@pgfornamentX{361}\def\@pgfornamentY{154}% 68
\or\def\@pgfornamentX{448}\def\@pgfornamentY{227}% 69
\or\def\@pgfornamentX{226}\def\@pgfornamentY{79}%  70
\or\def\@pgfornamentX{443}\def\@pgfornamentY{81}%  71
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  72
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  73
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  74
\or\def\@pgfornamentX{373}\def\@pgfornamentY{120}% 75
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  76
\or\def\@pgfornamentX{207}\def\@pgfornamentY{89}%  77
\or\def\@pgfornamentX{207}\def\@pgfornamentY{132}% 78
\or\def\@pgfornamentX{249}\def\@pgfornamentY{122}% 79
\or\def\@pgfornamentX{454}\def\@pgfornamentY{31}%  80
\or\def\@pgfornamentX{176}\def\@pgfornamentY{45}%  81
\or\def\@pgfornamentX{454}\def\@pgfornamentY{24}%  82
\or\def\@pgfornamentX{449}\def\@pgfornamentY{20}%  83
\or\def\@pgfornamentX{290}\def\@pgfornamentY{57}%  84
\or\def\@pgfornamentX{453}\def\@pgfornamentY{22}%  85
\or\def\@pgfornamentX{454}\def\@pgfornamentY{17}%  86
\or\def\@pgfornamentX{360}\def\@pgfornamentY{44}%  87
\or\def\@pgfornamentX{454}\def\@pgfornamentY{15}%  88
\or\def\@pgfornamentX{454}\def\@pgfornamentY{10}%  89
\fi%
}%
\makeatother
\endinput

==> pgflibraryam.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter

% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{133}\def\@pgfornamentY{48}%  2
\fi%
}%
% appels des motifs 
\def\pgf@@ornament#1{%
\begingroup
\def\i{\pgfusepath{clip}}
\let\o\pgfpathclose
\let\s\pgfusepathqfillstroke
\def\p ##1##2{\pgfqpoint{##1bp}{##2bp}}
\def\m ##1 ##2 {\pgfpathmoveto{\p{##1}{##2}}}
\def\l ##1 ##2 {\pgfpathlineto{\p{##1}{##2}}}
\def\r ##1 ##2 ##3 ##4 {\pgfpathrectangle{\p{##1}{##2}}{\p{##3}{##4}}}
\def\c ##1 ##2 ##3 ##4 ##5 ##6 {%
\pgfpathcurveto{\p{##1}{##2}}{\p{##3}{##4}}{\p{##5}{##6}}}%
\@@input am#1.pgf 
%\@nameuse{pgf@@am@#1}%
\endgroup}%
\makeatother
\endinput   

==> pgflibraryvectorian.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter
% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{134}\def\@pgfornamentY{48}%  2
\or\def\@pgfornamentX{130}\def\@pgfornamentY{65}%  3
\or\def\@pgfornamentX{133}\def\@pgfornamentY{133}% 4
\or\def\@pgfornamentX{129}\def\@pgfornamentY{146}% 5
\or\def\@pgfornamentX{134}\def\@pgfornamentY{148}% 6
\or\def\@pgfornamentX{136}\def\@pgfornamentY{135}% 7
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 8
\or\def\@pgfornamentX{79}\def\@pgfornamentY{105}% 9
\or\def\@pgfornamentX{80}\def\@pgfornamentY{99}%  10
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  11
\or\def\@pgfornamentX{136}\def\@pgfornamentY{136}% 12
\or\def\@pgfornamentX{136}\def\@pgfornamentY{236}% 13
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  14
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  15
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  16
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  17
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  18
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  19
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  20
\or\def\@pgfornamentX{70}\def\@pgfornamentY{58}%  21
\or\def\@pgfornamentX{34}\def\@pgfornamentY{61}%  22
\or\def\@pgfornamentX{68}\def\@pgfornamentY{55}%  23
\or\def\@pgfornamentX{79}\def\@pgfornamentY{76}%  24
\or\def\@pgfornamentX{80}\def\@pgfornamentY{88}%  25
\or\def\@pgfornamentX{59}\def\@pgfornamentY{120}% 26
\or\def\@pgfornamentX{101}\def\@pgfornamentY{98}%  27
\or\def\@pgfornamentX{52}\def\@pgfornamentY{102}% 28
\or\def\@pgfornamentX{65}\def\@pgfornamentY{65}%  29
\or\def\@pgfornamentX{63}\def\@pgfornamentY{64}%  30
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  31
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  32
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  33
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  34
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  35
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  36
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 37
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 38
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 39
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 40
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 41
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 42
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  43
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  44
\or\def\@pgfornamentX{385}\def\@pgfornamentY{64}%  45
\or\def\@pgfornamentX{453}\def\@pgfornamentY{97}%  46
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  47
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  48
\or\def\@pgfornamentX{163}\def\@pgfornamentY{61}%  49
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 50
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 51
\or\def\@pgfornamentX{248}\def\@pgfornamentY{197}% 52
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 53
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 54
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 55
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 56
\or\def\@pgfornamentX{207}\def\@pgfornamentY{103}% 57
\or\def\@pgfornamentX{228}\def\@pgfornamentY{116}% 58
\or\def\@pgfornamentX{204}\def\@pgfornamentY{102}% 59
\or\def\@pgfornamentX{451}\def\@pgfornamentY{189}% 60
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 61
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 62
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 63
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 64
\or\def\@pgfornamentX{132}\def\@pgfornamentY{166}% 65
\or\def\@pgfornamentX{177}\def\@pgfornamentY{175}% 66
\or\def\@pgfornamentX{80}\def\@pgfornamentY{155}% 67
\or\def\@pgfornamentX{361}\def\@pgfornamentY{154}% 68
\or\def\@pgfornamentX{448}\def\@pgfornamentY{227}% 69
\or\def\@pgfornamentX{226}\def\@pgfornamentY{79}%  70
\or\def\@pgfornamentX{443}\def\@pgfornamentY{81}%  71
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  72
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  73
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  74
\or\def\@pgfornamentX{373}\def\@pgfornamentY{120}% 75
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  76
\or\def\@pgfornamentX{207}\def\@pgfornamentY{89}%  77
\or\def\@pgfornamentX{207}\def\@pgfornamentY{132}% 78
\or\def\@pgfornamentX{249}\def\@pgfornamentY{122}% 79
\or\def\@pgfornamentX{454}\def\@pgfornamentY{31}%  80
\or\def\@pgfornamentX{176}\def\@pgfornamentY{45}%  81
\or\def\@pgfornamentX{454}\def\@pgfornamentY{24}%  82
\or\def\@pgfornamentX{449}\def\@pgfornamentY{20}%  83
\or\def\@pgfornamentX{290}\def\@pgfornamentY{57}%  84
\or\def\@pgfornamentX{453}\def\@pgfornamentY{22}%  85
\or\def\@pgfornamentX{454}\def\@pgfornamentY{17}%  86
\or\def\@pgfornamentX{360}\def\@pgfornamentY{44}%  87
\or\def\@pgfornamentX{454}\def\@pgfornamentY{15}%  88
\or\def\@pgfornamentX{454}\def\@pgfornamentY{10}%  89
\fi%
}%
\makeatother
\endinput
